Characterization of Lattice Properties Within Modal Extensions

This paper investigates the extension of lattice-based logics into modal languages. We observe that such extensions admit multiple approaches, as the interpretation of the necessity operator is not uniquely determined by the underlying lattice structure. The most natural interpretation defines necessity as the meet of the truth values of a formula across all accessible worlds -- an approach we refer to as the \textitnormal interpretation. We examine the logical properties that emerge under this and other interpretations, including the conditions under which the resulting modal logic satisfies the axiom K and other common modal validities. Furthermore, we consider cases in which necessity is attributed exclusively to formulas that hold in all accessible worlds.

==> eptcsdata.tex <==
\providecommand{\firstpage}{26}
\providecommand{\publicationstatus}{H. Barbosa, C. Ringeissen (Eds.): 20th International Symposium\\
on Logical and Semantic Frameworks with Applications\\
EPTCS 430, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.430.3}{10.4204/EPTCS.430.3}}
\pdfoutput=1

